A Strong Direct Sum Theorem for Distributional Query Complexity

Consider the expected query complexity of computing the $k$-fold direct product $f^{\otimes k}$ of a function $f$ to error $\varepsilon$ with respect to a distribution $\mu^k$. One strategy is to sequentially compute each of the $k$ copies to error $\varepsilon/k$ with respect to $\mu$ and apply the union bound. We prove a strong direct sum theorem showing that this naive strategy is essentially optimal. In particular, computing a direct product necessitates a blowup in both query complexity and error. Strong direct sum theorems contrast with results that only show a blowup in query complexity or error but not both. There has been a long line of such results for distributional query complexity, dating back to (Impagliazzo, Raz, Wigderson 1994) and (Nisan, Rudich, Saks 1994), but a strong direct sum theorem had been elusive. A key idea in our work is the first use of the Hardcore Theorem (Impagliazzo 1995) in the context of query complexity. We prove a new "resilience lemma" that accompanies it, showing that the hardcore of $f^{\otimes k}$ is likely to remain dense under arbitrary partitions of the input space.

==> AverageDepthOverview.tex <==

All the query algorithms that we consider will be randomized, so all probabilities and expectations are also with respect to the internal randomness of $T$.  

\begin{definition} Given a query algorithm $T : \bn\to\bits$  and a distribution $\mu$ over $\bn$, the {\sl expected depth of $T$ w.r.t.~$\mu$} is the quantity 
\[ \mathrm{Depth}^\mu(T) \coloneqq \Ex_{\bx \sim \mu}\big[\# \text{ queries }T\text{ makes on }\bx\big]. \]
\end{definition}

\begin{definition}[Distributional query complexity]
    For any function $f: \bits^n \to \bits$, distribution $\mu$ over $\bits$, and $\eps > 0$, the {\sl $\eps$-error distributional query complexity of $f$ w.r.t.~$\mu$} is the quantity: 
    \[ R^\mu_\eps(f) \coloneqq \min \big\{ \mathrm{Depth}^{\mu}(T)\colon \Prx_{\bx\sim \mu}[T(\bx)\ne f(\bx)]\le \eps\big\}.\]
  %  we use $R^\mu_{\eps}(f)$ to refer to the smallest $d \in \R$ for which there exists a algorithm $T$ for which,
   % \begin{equation*}
    %    \Prx_{\bx \sim \mu}[T(\bx) \neq f(\bx)] \leq \eps, \quad\quad\text{and}\quad\quad\Ex_{\bx \sim \mu}[\# \text{ queries }T\text{ makes on }\bx] \leq d.
    %\end{equation*}
    %Note that both expectations are over the randomness of $\bx$ and in the internal randomness of $T$.
\end{definition}

\paragraph{Notation.} For a function $f : \bn\to\bits$, we write $f^{\otimes k} : (\bn)^k \to \bits^k$ to denote its direct product: 
\[ f^{\otimes k}(X) \coloneqq  (f(X^{(1)}),\ldots,f(X^{(k)})).\]
We use $X \in (\bn)^k$ to denote an input to $f^{\otimes k}$, $X^{(i)} \in \bn$ to denote its $i^{th}$ block, and $x\in \bn$ to denote a generic input to $f$. 
%\begin{theorem}[Dream theorem: Strong direct product theorem for $R^\mu(f)$]\gnote{To discuss: We will only be able to handle constant $\gamma$. DP theorems with exponentially small $\gamma$ don't hold for expected depth (or expected amount of any resource).}
 %   For any function $f:\bits^n \to \bits$, $k \in \N$, distribution $\mu$, and $\gamma,\delta > 0$,
  %  \begin{equation*}
   %     R_{\frac1{2}-\gamma}^{\mu^k}(f^{\otimes k}) \ge \Omega(k) \cdot R^\mu_{\delta}(f) \quad \text{where} \quad k = \Theta\left(\frac{\log(1/\gamma)}{\delta}\right).
   % \end{equation*}
%\end{theorem}
%The semantics of $k$ is that it satisfies $(1-\delta)^k \le \gamma.$ 
%The goal of this note is to sketch a proof that for any $\eps \geq 0.01$,
%\begin{equation*}
%    R_\eps^{\mu^k}(f^{\otimes k}) \geq \Omega\paren*{\frac{k}{\log (k/\eps)}} \cdot R^\mu_{\Omega(\eps/k)}(f).
%\end{equation*}
%The moment we use the hardcore measure Lemma, we lose the $\log k$ factor. It's possible the we can get a statement like the above for all $\eps$ with a tighter analysis.

%Relatedly, we think we can show that for every $\delta$,  

\section{Preliminaries} 

\subsection{The hardcore lemma}
 

\begin{definition}[Hardcore measure]
    \label{def:hardcore measure}
    We say $H:\bits^n \to [0,1]$ is a {\sl $(0.1,d)$-hardcore measure for $f:\bits^n \to \bits$ w.r.t. $\mu$ of density $\delta$} if: 
    \begin{enumerate}
        \item Density: $\ds \Ex_{\bx\sim \mu}[H(\bx)] = \delta.$
        \item Hardness: For all query algorithms $T$ with $\mathrm{Depth}^\mu(T) \le d$,
    \begin{equation*}
        \Big| \Ex_{\bx \sim \mu}[ f(\bx) T(\bx) H(\bx)]\Big|  \leq 0.1 \cdot \Ex_{\bx \sim \mu}[H(\bx)]
    \end{equation*} 
    \end{enumerate} 
\end{definition}

\begin{remark} For the special case where $H : \bn \to \zo$ is the indicator of a {\sl set} (as in the traditional hardcore set lemma as used in Yao's XOR lemma), the above are equivalent to the more familiar looking: 
\begin{enumerate}
    \item {\it Density:} $\ds \Prx_{\bx\sim \mu}[\bx \in H] = \delta.$
    \item {\it Hardness:} $\ds \Big|\Ex_{\bx \sim \mu}[f(\bx) T(\bx) \mid \bx\in H]\Big|  \leq 0.1$ 
\end{enumerate}

\end{remark}

The traditional hardcore set lemma assumes that $\mu$ is the uniform distribution; for general distributions $\mu$ we have to allow for $H$ to be a measure instead of a set.  



\begin{theorem}[The hardcore lemma for $R^\mu(f)$]
For every $f : \bn \to \bits$ be such that $R^\mu_\delta(f) \ge d$ w.r.t.~a distribution $\mu$, there exists a $(0.1,\Omega(d/\log(1/\delta))$-hardcore measure for $f$ w.r.t.~$\mu$ of density~$\delta$.
\end{theorem} 
\section{Total hardcore density and total hardcore advantage} 

Let $T$ be a query algorithm for $f^{\otimes k}: (\bn)^k \to \bits$ and $H : \bn\to [0,1]$ be a hardcore measure for $f$. For every leaf $\ell$ of $T$, we define two key quantities, the total hardcore density $\Delta(\ell)$ and total advantage $A(\ell)$ at that leaf:  

\lnote{Proposal for more readable notation: $A(\ell) \to \mathrm{Adv}_H(\ell)$ and $\Delta(\ell) \to \mathrm{Dens}_H(\ell)$.}
\lnote{Let's formalize and explain why $\mathrm{Dens}_H(\ell)$ is a good proxy for the hardcore density of $(f^{\otimes k})_\ell$.}

\begin{definition}[Total hardcore density]
    For a leaf $\ell$ of $T$, the hardcore density at leaf $\ell$ in the $i^{\text{th}}$ block is
    \begin{equation*}
        \delta(\ell, i) \coloneqq \Ex_{\bX \sim \ell}[H(\bX^{(i)})].
    \end{equation*}
    The total hardcore density at leaf $\ell$ is defined as
    \begin{equation*}
        \Delta(\ell) \coloneqq \sum_{i \in [k]} \delta(\ell, i).
    \end{equation*}
\end{definition} 

Similarly: 


\begin{definition}[Total hardcore advantage]
    For a leaf $\ell$ of $T$, the \textit{hardcore advantage} at leaf $\ell$ in the $i^{th}$ block is
    \begin{equation*}
        \alpha(\ell,i)\coloneqq \Big|\Ex_{\bX\sim \ell}\big[f(\bX^{(i)}) H(\bX^{(i)})\big]\Big|
    \end{equation*}
    and the total hardcore advantage at leaf $\ell$ is
    \begin{equation*}
        A(\ell)\coloneqq \sum_{i\in [k]} \alpha(\ell, i).
    \end{equation*}
\end{definition}

Note that 
\[ \Big|\Ex_{\bX\sim \ell}\big[f(\bX^{(i)}) H(\bX^{(i)})\big]\Big| = \max_{y\in \bits} \Big\{ \Ex_{\bX\sim \ell}\big[f(\bX^{(i)}) y H(\bX^{(i)})\big] \Big\}, \]
i.e.~among the inputs that reach $\ell$, this is  the advantage achievable on the $i^{th}$ block w.r.t.~$H$ by labeling~$\ell$ with the best constant $\in \bits$.  Therefore: 

\begin{fact} 
\label{fact:semantics of A} 
For any tree $T$,
\[ \sum_{i=1}^k \underbrace{\Big| \Ex_{\bX\sim \mu^k}\big[ f(\bX^{(i)})T(\bX^{(i)})H(\bX^{(i)})\big] \Big|}_{\textnormal{Advantage of $T$ on the $i^{th}$ block w.r.t.~$H$}} \le \Ex_{\bell\sim T}[A(\bell)],\]   with equality iff $T$ labels its leaves optimally. 
\end{fact}

\subsection{Key property of total hardcore density: Many leaves have high total hardcore density} 
Suppose $H$ is a hardcore measure of density $\delta$. 
\begin{fact}[Conservation of hardcore density] 
\label{fact:conservation of hardcore density} For every block $i\in [k]$,
\[ \Ex_{\bell\sim T}[\delta(i,\bell)] = \Ex_{\bell\sim T}\Big[ \Ex_{\bX \sim \bell}[H(\bX^{(i)})]\Big] = \Ex_{\bX \sim \mu^k}[H(\bX^{(i)})] = \delta.\]
Consequently, the expected total hardcore density is \[ \Ex_{\bell\sim T}[\Delta(\bell)] = \sum_{i=1}^k \Ex_{\bX\sim\mu^k}[H(\bX^{(i)})] = \delta k \]  
\end{fact} 

We are interested in how this expectation is achieved. \lnote{To do: elaborate on the following in proof overview.}
\begin{itemize}
\item[$\circ$] Dream scenario: $\mathrm{Dens}_H(\ell) = \delta k$ for all $\ell \in T$. 
\item[$\circ$] Bad case for us:  $\mathrm{Dens}_H(\ell) = k$ for $\delta$-fraction of $\ell\in T$, and $\mathrm{Dens}_H(\ell) = 0$ otherwise.   
\end{itemize}
The following lemma tells us that the random variable $\Delta(\bell)$ is somewhat well-concentrated around its expectation: 


\gray{ \begin{lemma}[Many leaves have high total hardcore density]\lnote{This is subsumed by the next lemma, right? If so, let's delete.}
\label{lem:concentration of hardcore density} 
    For any tree $T:(\bits^n)^k \to \bits$, distribution $\mu$ over $\bits^n$, and hardcore measure $H:\bits^n \to [0,1]$ with density $\delta$,\gnote{Todo, check if this is what Paley–Zygmund gives}
    \begin{equation*}
        \Prx_{\bell \sim T}\bracket*{\Delta(\bell) \geq \frac{\delta k}{2}} \geq \frac{\min(1, \delta k)}{8}.
    \end{equation*}
    Similarly, if $\delta k \geq 8$,\gnote{This is via Chebyshev, and we may end up sticking to the regime of $\delta k$ is a constant.}
    \begin{equation*}
        \Prx_{\bell \sim T}\bracket*{\Delta(\bell) \geq \frac{\delta k}{2}} \geq \frac{1}{2}.
    \end{equation*}
\end{lemma}

For example, \Cref{lem:concentration of hardcore density} rules out the possibility that $\E[\Delta(\bell)] = \delta k$ is achieved by having a $\delta$ fraction of leaves $\ell$ satisfy $\Delta(\ell) = k$ and the remaining $1-\delta$ fraction satisfy $\Delta(\ell) = 0$. }


\begin{lemma}[More fine-grained understanding understanding of hardcore density]\gnote{This may give a cleaner/tighter proof than the above strategy}
    \label{lem:convex-leaves}
    Let $\bz \sim \Bin(\delta, k)$. Then, for any convex function $f:\R \to \R$,
    \begin{equation*}
        \Ex_{\bell \sim T}[f(\Delta(\bell))] \leq \Ex_{\bz}[f(\bz)].
    \end{equation*}
    For our applications, we can use the MGF: For any $\lambda \in R$,
    \begin{equation*}
        \Ex_{\bell \sim T}[e^{\lambda\Delta(\bell)}] \leq (1 + \delta(e^{\lambda}-1))^k.
    \end{equation*}
\end{lemma}
\begin{proof}
    For any $X \in (\bits^n)^k$, let $\Delta(X) = \sum_{i \in [k]}\Delta(X^{(i)})$.\lnote{What is $\Delta(X^{(i)})?$ Is it $\Ind[X^{(i)}\in H]?$} Then, by Jensen's inequality,
    \begin{equation*}
        \Ex_{\bell \sim T}[f(\Delta(\bell))] =  \Ex_{\bell \sim T}[f(\Ex_{\bX \sim \bell}[\Delta(\bX)])] \leq \Ex_{\bell \sim T}[\Ex_{\bX \sim \bell}[f(\Delta(\bX))]].
    \end{equation*}
    The Lemma follows from the distribution of $\Delta(\bX)$ being that of $\Bin(\delta, k)$.
\end{proof}
\subsection{Key property of total hardcore advantage: depth amplification} 

\begin{lemma}[Depth amplification]
\label{lem:expectation of total hardcore advantage} 
    If $H$ is a $(0.1,d)$-hardcore measure for $f:\bits^n \to \bits$ w.r.t. $\mu$ and $T:(\bits^n)^k \to \bits$ makes at most $dk$ queries on average
\[         \label{eq:avg-advantage}
        \Ex_{\bell \sim T}[A(\bell)] \leq 0.1 \Ex_{\bell\sim T}[\Delta(\bell)] = 0.1\delta k.
    \]
\end{lemma}

Recalling what it means for $H$ to be a hardcore measure (\Cref{def:hardcore measure}) and the semantics of $\E[A(\bell)]$ (\Cref{fact:semantics of A}), this lemma says that if $f$ and $H$ are such that any $d$-query algorithm $T_{\textnormal{small}} : \bn\to\bits$ satisfies  
    \begin{equation*}
        \underbrace{\Big| \Ex_{\bx \sim \mu}[ f(\bx) T_{\textnormal{small}}(\bx) H(\bx)]\Big|}_{\textnormal{Hardcore advantage}}  \leq 0.1 \cdot \underbrace{\Ex_{\bx \sim \mu}[H(\bx)]}_{\textnormal{Hardcore density}}
    \end{equation*} 
then any $dk$-query algorithm $T_{\textnormal{large}} : (\bn)^k \to \bits$ satisfies 
\[ \underbrace{\sum_{i=1}^k \Big| \Ex_{\bX\sim \mu^k}\big[ f(\bX^{(i)})T_{\textnormal{large}}^{(i)}(\bX) H(\bX^{(i)})\big] \Big|}_{\textnormal{Total hardcore advantage}} \le 0.1 \cdot \underbrace{\sum_{i=1}^k \Ex_{\bX\sim\mu^k}[H(\bX^{(i)})]}_{\Ex_{\bell\sim T}[\Delta(\bell)] = \textnormal{Total hardcore density}}. \]

Note that the query complexity of $T_{\textnormal{large}}$ is allowed to be a factor of $k$ larger than that of $T_{\textnormal{small}}$, and yet the ratio of hardcore advantage to hardcore density remains the same.  

We prove this lemma via contrapositive: We show that if there is a $dk$-query algorithm $T_{\textnormal{large}}$ that violates~\Cref{eq:avg-advantage}, we can extract a $d$-query algorithm $T_{\textnormal{small}}$ that achieves too much advantage for elements of the hardcore measure, violating \Cref{def:hardcore measure}.%\lnote{To discuss: Is this basically what's done in Theorem 4.3 of Ben-David--Kothari?}


We'll also use the following simple fact.
\begin{fact}[Boundedness of total hardcore advantage]
    For any leaf $\ell$, $0\leq A(\ell) \leq \Delta(\ell)$.
\end{fact}



\section{Success probability in terms of $\Delta(\ell)$'s and $A(\ell)$'s} 

\begin{lemma}[Best error of a tree for direct product]
\label{lem:success in terms of Delta and A} 
    For any function $f: \bits^n \to \bits$, distribution $\mu$ over $\bits^n$, $H:\bits^n \to [0,1]$, and tree $T:(\bits^n)^k \to \bits^k$,
    \begin{equation*}
        \Prx_{\bX \sim \mu^k}[T(\bX) = f^{\otimes k}(\bX)] \leq \Ex_{\bell \sim T}\bracket*{\exp\paren*{ -\frac{\Delta(\bell) - A(\bell)}{2}}}.
    \end{equation*}
\end{lemma}


\paragraph{Intuition for why~\Cref{lem:success in terms of Delta and A} implies~\Cref{thm:main}.}  Recall that~\Cref{fact:conservation of hardcore density} says that $\E[\Delta(\bell)] = \delta k$ and~\Cref{lem:expectation of total hardcore advantage} says that $\E[A(\bell)] \le 0.1 \delta k$. These suggest that 
\[ \Pr[T(\bX) = f^{\otimes k}(\bX)] \le \exp(-\Omega(\delta k)).\]
Jensen's goes the wrong way, i.e.~we do {\sl not} have 
\[ \Ex_{\bell \sim T}\bracket*{\exp\paren*{ -\frac{\Delta(\bell) - A(\bell)}{2}}} \le 
\exp\left(-\frac{\Ex_{\bell\sim T}[\Delta(\bell)-A(\bell)]}{2}\right),\] 
but  using~\Cref{lem:concentration of hardcore density} we'll show that this is morally correct. 

\medskip 

\paragraph{Alternative proof strategy.} We know that $\Delta(\ell) - A(\ell) \geq 0$. Therefore, the error can also be written as
\begin{equation*}
     \Prx_{\bX \sim \mu^k}[T(\bX) = f^{\otimes k}(\bX)] \leq \Ex_{\bell \sim T}\bracket*{\exp\paren*{ -\max\paren*{0,\frac{\Delta(\bell) - A(\bell)}{2}}}}.
\end{equation*}
We observe that the function $h(x) = e^{-\max(0, x)}$ is $1$-Lipschitz (because it's derivative is at most $1$), so we can bound,
\begin{align*}
    \Prx_{\bX \sim \mu^k}[T(\bX) = f^{\otimes k}(\bX)] &\leq \Ex_{\bell \sim T}\bracket*{\exp\paren*{ -\max\paren*{0,\frac{\Delta(\bell)}{2}}} + \frac{A(\bell)}{2}} \\
    &= \Ex\bracket*{e^{-1/2 \cdot \Delta(\bell)}} + \frac{1}{2} \cdot \Ex[A(\bell)] \\
    &\leq (1 + \delta(e^{-1/2}-1))^k + 0.05\delta k \tag{\Cref{lem:convex-leaves,lem:expectation of total hardcore advantage}}\\
    &\leq (1 -0.39\delta)^k + 0.05\delta k
\end{align*}
For example, if $\delta k \leq 5$, the above is at most\gnote{If we actually include this, check my math} $1 - 0.12 \delta k$.



%\section{XOR lemma} 
%A similar results holds for direct sum.
%\begin{lemma}[Best error of a tree for direct sum (XOR lemma)]
%    For any function $f: \bits^n \to \bits$, distribution $\mu$ over $\bits^n$, $H:\bits^n \to [0,1]$, and tree $T:(\bits^n)^k \to \bits$,
%    \begin{equation*}
%        \Prx_{\bx \sim \mu^k}[T(\bx) = f^{\oplus k}(\bx)] \leq \frac{1}{2} + \frac{1}{2} \cdot\Ex_{\bell \sim T}\bracket*{\exp\paren*{ -\big(\Delta(\bell) - A(\bell)\big)}}.
 %   \end{equation*}
%\end{lemma}

==> blais-brody.tex <==
\section{Implications for randomized query complexity}
\label{sec:randomized query complexity}
%In this section, we use \Cref{thm:main-formal} to recover a result due to \cite{BB19} which shows that randomized query complexity admits a strong direct product theorem. In an analogous fashion, we use \Cref{thm:main-xor} to recover a result due to \cite{BKLS20} which shows that randomized query complexity admits a strong XOR lemma.

% It will be convenient in this section for us to regard $\overline{\mathrm{Depth}}^\mu(f,\eps)$ as minimum expected depth of a \textit{deterministic} algorithm computing $f$ to error $\eps$. 

\paragraph{Randomized query complexity.}{For a randomized query algorithm $\bT$ and a function $f:\bits^n\to\bits$, we say that $\bT$ has error $\eps$ if $\max_{x\in\bits^n}\Pr_{\bT}[\bT(x)\neq f(x)]\le \eps$ and query complexity $q$ if $\max_{x\in \bits^n}\E_{\bT}[\# \text{ queries to }x]\le q$. The $\eps$-error randomized query complexity of $f$ is the minimum query complexity of any randomized algorithm which computes $f$ with error $\eps$. We write $\overline{\mathrm{R}}(f,\eps)$ to denote the $\eps$-error randomized query complexity of $f$.
}


The authors in \cite{BB19} show that $\overline{\mathrm{R}}$ admits the following direct product theorem: 

\begin{theorem}[Strong direct product theorem for randomized query complexity \cite{BB19}]
\label{thm:blais-brody}
    For every $f:\bits^n\to\bits$, $\eps<\frac{1}{20}$, and $k\ge 2$,
    $$
    \overline{\mathrm{R}}(f^{\otimes k},\eps)\ge \Omega(k)\cdot\overline{\mathrm{R}}\big(f, \tfrac{\eps}{k}\big).
    $$
\end{theorem}
Similarly, the authors in \cite{BKLS20} show that $\overline{\mathrm{R}}$ admits the following strong XOR lemma:

\begin{theorem}[Strong XOR lemma for randomized query complexity \cite{BKLS20}]
\label{thm:brody-et-al}
    For every $f:\bits^n\to\bits$, small enough constant $\eps >0$, and $k\ge 2$,
    $$
    \overline{\mathrm{R}}(f^{\oplus k},\eps)\ge \Omega(k)\cdot \overline{\mathrm{R}}(f,\tfrac{\eps}{k}). 
    $$
\end{theorem}

Our strong direct product theorem (\Cref{thm:main-formal}) and strong XOR lemma (\Cref{thm:main-xor})  
for distributional query complexity can recover these results up to logarithmic factors in $k$. First note that the randomized query complexity of a function is at least its distributional query complexity: any randomized algorithm $\bT$ satisfying $\Pr_{\bT}[\bT(x)\neq f(x)]\le \eps$ and $\E_{\bT}[\# \text{ queries to }x]\le q$ for all $x$ also satisfies $\Ex_{\bx\sim \mu}[\Pr_{\bT}[\bT(x)\neq f(x)]]\le \eps$ and $\Ex_{\bx\sim \mu}[\E_{\bT}[\# \text{ queries to }\bx]]\le q$ for all distributions $\mu$. 

\begin{fact}
\label{fact:pointwise-r-vs-avg-depth}
    For all $f:\bits^n\to\bits$, distributions $\mu$ over $\bits^n$, and $\eps>0$, $\overline{\mathrm{R}}(f,\eps)\ge \overline{\mathrm{Depth}}^\mu(f,\eps)$. 
\end{fact}

Next, we use the following version of Yao's minimax theorem which shows that the randomized query complexity of a function is at most its distributional query complexity, up to constants. 

\begin{theorem}[\cite{Vere98}]
\label{thm:vereshchagin}
    For all $f:\bits^n\to\bits$ and $\eps>0$, there exists a distribution $\mu$ such that
    $$
    \overline{\mathrm{R}}(f,\eps)\le 4\cdot \overline{\mathrm{Depth}}^\mu\big(f,\tfrac{\eps}{4}\big).
    $$
\end{theorem}
In more detail, \cite{Ver98} shows that there is a distribution $\mu$ such that $\overline{\mathrm{R}}(f,\eps)$ is at most $2 q$ where $q$ is the distributional query complexity of computing $f$ with \textit{deterministic} algorithms to error $\eps/2$ over~$\mu$. By Markov's inequality, any \textit{randomized} algorithm with error $\eps$ and expected query cost $q$ can be converted to a deterministic one with error $2\eps$ and expected query cost $2q$ (see e.g. the argument in \Cref{claim:connect-det-rand}). \Cref{thm:vereshchagin} then follows.

% The main lemma we require relates expected query complexity to distributional query complexity with aborts.

% \begin{lemma}
% \label{lem:avg-depth-to-aborts}
%     For any $\alpha,\beta>0$ satisfying $\alpha+\beta\le 1$, we have that
%     $$
%     \overline{\mathrm{Depth}}^\mu(f,\eps)\ge \alpha^2\cdot \mathrm{Depth}_{\Pr[\bot]\le \alpha}^\mu (f,\frac{\eps}{\beta}).
%     $$
% \end{lemma}

% \begin{proof}
% Let $d=\overline{\mathrm{Depth}}^\mu(f,\eps)$ and let $A$ be a query algorithm satisfying $d=\E[\#\text{ queries made to }\bx\text{ by }A]$ and $\Pr[A(\bx)\neq f(\bx)]\le \eps$. Since $A$ is a randomized query algorithm, it can be viewed as a distribution $\mathcal{T}$ over (deterministic) decision trees. For a decision tree $T$, let $\mathrm{error}(T)$ denote the error $T$ makes in computing $f$ over $\mu$ and let $\Delta^\mu(T)$ denote the average depth of $T$ for $\bx\sim\mu$. Then by assumption, we have $\Ex_{\bT\sim\mathcal{T}}[\mathrm{error}(\bT)]\le \eps$ and $\Ex_{\bT\sim\mathcal{T}}[\Delta^\mu (\bT)]=d$ so by Markov:
% $$
% \Prx_{\bT\sim\mathcal{T}}[\mathrm{error}(\bT)>\eps/\beta]< \beta\quad\text{and}\quad \Prx_{\bT\sim\mathcal{T}}[\Delta^\mu (\bT)>d/\alpha]<\alpha.
% $$
% Therefore, by a union bound, there is some fixed $T$ such that $\mathrm{error}(T)\le \eps/\beta$ and $\Delta^\mu (T)\le d/\alpha$. Let $T'$ be the query algorithm which simulates $T$ but aborts if $T$ makes more than $d/\alpha^2$ queries. Then the probability that $T'$ aborts is at most $\alpha$ by Markov. Since $T'$ has depth $d/\alpha^2$ and has error at most $\eps/\beta$, this shows that $d/\alpha^2\ge {\mathrm{Depth}^\mu}_{\Pr[\bot]\le \alpha}(f,\eps/\beta)$.
% \end{proof}

\subsection{Recovering the strong direct product theorem and the XOR lemma for randomized query complexity}

\paragraph{Strong direct product theorem.}
Combining the above observations, 
\begin{align*}
    \overline{\mathrm{R}}(f^{\otimes k},\eps)&\ge \overline{\mathrm{Depth}}^{\mu^k}(f^{\otimes k},\eps)\tag{\Cref{fact:pointwise-r-vs-avg-depth}}\\
    &\ge \Tilde{\Omega}(k)\cdot \overline{\mathrm{Depth}}^\mu(f,\Theta(\tfrac{\eps}{k}))\tag{\Cref{thm:main-formal}}\\
    &\ge \Tilde{\Omega}(k)\cdot \overline{\mathrm{R}}(f,\Theta(\tfrac{\eps}{k}))\tag{\Cref{thm:vereshchagin}}
\end{align*}
where $\mu$ denotes the hard distribution from \Cref{thm:vereshchagin}. Finally, by success amplification we have $\overline{\mathrm{R}}(f,\tfrac{\eps}{k})\le O(\overline{\mathrm{R}}(f,\Theta(\tfrac{\eps}{k})))$ which completes the proof.\qed


\paragraph{Strong XOR lemma.} Similarly, 
\begin{align*}
    \overline{\mathrm{R}}(f^{\oplus k},\eps)&\ge \overline{\mathrm{Depth}}^{\mu^k}(f^{\oplus k},\eps)\tag{\Cref{fact:pointwise-r-vs-avg-depth}}\\
    &\ge \Tilde{\Omega}(k)\cdot \overline{\mathrm{Depth}}^\mu(f,\Theta(\tfrac{\eps}{k}))\tag{\Cref{thm:main-xor}}\\
    &\ge\Tilde{\Omega}(k)\cdot \overline{\mathrm{R}}(f,\Theta(\tfrac{\eps}{k}))\tag{\Cref{thm:vereshchagin}}
\end{align*}
where $\mu$ denotes the hard distribution from \Cref{thm:vereshchagin}.  Again by success amplification we have $\overline{\mathrm{R}}(f,\frac{\eps}{k})\le O(\overline{\mathrm{R}}(f,\Theta(\tfrac{\eps}{k})))$ which completes the proof.\qed



% \begin{align*}
%     \overline{R}(f,\frac{8\eps}{k})&\le 2\cdot \mathrm{Depth}^\mu_{\Pr[\bot]\le \frac{1}{4}}(f,\frac{2\eps}{k})\tag{\Cref{claim:pointwise-r-to-aborts}}\\
%     &\le 32\cdot \overline{\mathrm{Depth}}^\mu(f,\frac{\eps}{k})\tag{\Cref{lem:avg-depth-to-aborts}}.\\
% \end{align*}
% By success amplification, we have $\overline{R}(f,\frac{\eps}{k})\le O(\overline{R}(f,\frac{8\eps}{k}))$. Therefore, we can write
% \begin{align*}
%     \overline{R}(f^{\otimes k},\eps)&\ge \overline{\mathrm{Depth}}^{\mu^k}(f^{\otimes k},\eps)\tag{\Cref{fact:pointwise-r-vs-avg-depth}}\\
%     &\ge \Tilde{\Omega}(k)\cdot \overline{\mathrm{Depth}}^\mu(f,\frac{\eps}{k})\\
%     &\ge  \Tilde{\Omega}(k)\cdot \overline{R}(f,\frac{\eps}{k})
% \end{align*}
% which completes the proof. 

% \begin{align*}
%    \overline{R}(f^{\otimes k},\eps)&\ge \overline{\mathrm{Depth}}^{\mu^k}(f^{\otimes k},\eps)\\
%    &\ge \Tilde{\Omega}(k)\cdot \overline{\mathrm{Depth}}^\mu(f,\frac{\eps}{k})\\
%    &\ge \Tilde{\Omega}(k)\cdot \mathrm{Depth}_{\Pr[\bot]\le \alpha}^\mu (f,\frac{\eps}{k})\\
%    &\ge \Tilde{\Omega}(k)\cdot \overline{R}(f,\frac{\eps}{k}).
% \end{align*}
